Natural Strategic Abilities in Voting Protocols

Security properties are often focused on the technological side of the system. One implicitly assumes that the users will behave in the right way to preserve the property at hand. In real life, this cannot be taken for granted. In particular, security mechanisms that are difficult and costly to use are often ignored by the users, and do not really defend the system against possible attacks. Here, we propose a graded notion of security based on the complexity of the user's strategic behavior. More precisely, we suggest that the level to which a security property $\varphi$ is satisfied can be defined in terms of (a) the complexity of the strategy that the voter needs to execute to make $\varphi$ true, and (b) the resources that the user must employ on the way. The simpler and cheaper to obtain $\varphi$, the higher the degree of security. We demonstrate how the idea works in a case study based on an electronic voting scenario. To this end, we model the vVote implementation of the \Pret voting protocol for coercion-resistant and voter-verifiable elections. Then, we identify "natural" strategies for the voter to obtain receipt-freeness, and measure the voter's effort that they require. We also look at how hard it is for the coercer to compromise the election through a randomization attack.

==> complexity.tex <==
\section{Measuring complexity}

In this section we consider the strategies defined in Section \ref{sec:strats} and measure their complexities by considering the metric described in \ref{sec:methodology}.

We start with the Natural Strategy \ref{mainstrat}. Here, we have eight guarded commands in which the command (4) costs 3 since we have three symbols (two atoms plus the disjunction), while the other guarded commands cost 1, so the total complexity is 10.

In Natural Strategy \ref{mainstratwithchecks}, we introduce the verification of $check1$ and $check3$. To do this we add two new guarded commands (5) and (6), and we update (1) by adding the control of a counter to determine if $check1$ is done or not. Here, we have a total complexity of 14. 

In Natural Strategy \ref{mainstratcheck2}, we consider the extension of Natural Strategy \ref{mainstrat} in which we refine the atomic step $check2$ in accordance with Figure \ref{fig:votcheck2}. In particular, we have twelve guarded commands all define with a single atom but (8) in which we have a disjunction of two atoms. So, the total complexity is 14.

To conclude, in Natural Strategy \ref{mainstratcheck2ref}, we consider the extension of Natural Strategy \ref{mainstratcheck2} in which we adopt the additional refinement of $check2$ described in Figures \ref{fig:checksn} and \ref{fig:checkpp}. In this natural strategy we have sixteen guarded commands in which (6) and (9) are conjunctions of two atoms, (14) is a disjunction of four atoms, and all the other guarded commands are defined with a single atom. Therefore, the complexity of Natural Strategy \ref{mainstratcheck2ref} is $3 \cdot 2 + 7 + 13 = 26$.
 
